TokenVerse: Versatile Multi-concept Personalization in Token Modulation Space

We present TokenVerse -- a method for multi-concept personalization, leveraging a pre-trained text-to-image diffusion model. Our framework can disentangle complex visual elements and attributes from as little as a single image, while enabling seamless plug-and-play generation of combinations of concepts extracted from multiple images. As opposed to existing works, TokenVerse can handle multiple images with multiple concepts each, and supports a wide-range of concepts, including objects, accessories, materials, pose, and lighting. Our work exploits a DiT-based text-to-image model, in which the input text affects the generation through both attention and modulation (shift and scale). We observe that the modulation space is semantic and enables localized control over complex concepts. Building on this insight, we devise an optimization-based framework that takes as input an image and a text description, and finds for each word a distinct direction in the modulation space. These directions can then be used to generate new images that combine the learned concepts in a desired configuration. We demonstrate the effectiveness of TokenVerse in challenging personalization settings, and showcase its advantages over existing methods. project's webpage in https://token-verse.github.io/

==> figures/limitation_ablation_minipage.tex <==
\begin{figure*}[t]
    \centering
    \scriptsize
    \begin{tabular}{c c}
        \begin{minipage}[b]{0.5\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/ablation3.pdf}
            \caption{\textbf{Ablations.} The top row lists all the concepts used to generate the result images. Each column, (a) to (d), shows the results of our method as additional components are progressively integrated.}
            \label{fig:ablation_fig}
        \end{minipage} &
        \begin{minipage}[b]{0.5\linewidth}
            \centering
            \includegraphics[width=\linewidth]{images/limitation2.pdf}
            \caption{\textbf{Limitations.} 
            Concept images are shown in the top row, with the generated images using TokenVerse below in each case. While our method supports both disentangled learning and multi-concept composition, limitations remain. (a) Rare blending can occur in specific combinations due to independent training of concepts; We provide analysis and mitigations in the SM. (b) Challenges arise with concepts sharing the same name identifier, which can be mitigated by using distinct terms. (c) Certain incompatible combinations, such as a doll with tiny limbs in a complex pose, may result in undesired outputs.
            } 
            \label{fig:limitation_fig}
        \end{minipage} \\
    \end{tabular}
\end{figure*}

